Investigating the Role of Instruction Variety and Task Difficulty in Robotic Manipulation Tasks

Evaluating the generalisation capabilities of multimodal models based solely on their performance on out-of-distribution data fails to capture their true robustness. This work introduces a comprehensive evaluation framework that systematically examines the role of instructions and inputs in the generalisation abilities of such models, considering architectural design, input perturbations across language and vision modalities, and increased task complexity. The proposed framework uncovers the resilience of multimodal models to extreme instruction perturbations and their vulnerability to observational changes, raising concerns about overfitting to spurious correlations. By employing this evaluation framework on current Transformer-based multimodal models for robotic manipulation tasks, we uncover limitations and suggest future advancements should focus on architectural and training innovations that better integrate multimodal inputs, enhancing a model's generalisation prowess by prioritising sensitivity to input content over incidental correlations.

==> tables/difficulty-no-instruct.tex <==
\begin{table}[tb]
\centering
\footnotesize
\sisetup{table-format=2.1}
\renewcommand{\arraystretch}{1.25}
\begin{tabularx}{\linewidth}{X SSSS @{}}
\toprule
& {L1} & {L2} & {L3} & {L4} \\
\midrule
\multicolumn{5}{@{}l}{\textit{Distracting}} \\
Cross-Attn + Obj-Centric & 33.0 & 32.2 & 21.0 & 21.9 \\
Cross-Attn + Patches &6.7 & 7.3 & 2.4 & 2.6 \\
Concatenate + Obj-Centric  & 5.9 & 4.5 & 1.2 & 0.6 \\
Concatenate + Patches &  6.5 & 6.7 & 3.4 & 1.6 \\
\midrule[0.2pt] 
\multicolumn{5}{@{}l}{\textit{Extreme}} \\
Cross-Attn + Obj-Centric &  15.2 & 15.5 & 17.4 & 11.2 \\
Cross-Attn + Patches & 5.7 & 4.6 & 2.7 & 4.6 \\
Concatenate + Obj-Centric  & 4.5 & 3.3 & 2.0 & 2.2 \\
Concatenate + Patches & 3.9 & 4.1 & 2.7 & 7.4 \\
\midrule[0.2pt] 
\multicolumn{1}{@{}l}{\textit{Extremely Distracting}} \\
Cross-Attn + Obj-Centric &10.1 & 8.7 & 8.7 & 10.9 \\
Cross-Attn + Patches & 2.9 & 2.8 & 0.4 & 3.6 \\
Concatenate + Obj-Centric  & 4.3 & 4.3 & 2.0 & 1.4 \\
Concatenate + Patches & 1.7 & 1.6 & 0.4 & 1.2 \\
\bottomrule
\end{tabularx}
\caption{Difficulty + No Prompt. Trained Para. No Mistakes allowed.}
\label{tab:perf-difficulty-no-instruct}
\end{table}


==> tables/gdg-on-orig.tex <==


\begin{table}[tb]
\centering
\footnotesize
\sisetup{table-format=2.1}
\renewcommand{\arraystretch}{1.3}
\begin{tabularx}{\linewidth}{X SSSS @{}}
\toprule
& {L1} & {L2} & {L3} & {L4} \\
\midrule
\multicolumn{5}{@{}l}{\textit{Train Orig; Eval Orig + }\GDGTokens} \\
Cross-Attn + Obj-Centric & \bfseries 57.9 & \uline{55.0} & \uline{39.1} & 16.9 \\
Cross-Attn + Patches & 44.3 & 40.9 & 29.6 & 11.4\\
Concatenate + Obj-Centric& \uline{55.9} & \bfseries 55.5 & \bfseries 42.0 & \bfseries 26.2 \\
Concatenate + Patches& 44.0 & 43.0 & 31.7 & \uline{21.6} \\
\midrule[0.2pt] 
\multicolumn{5}{@{}l}{\textit{Train Orig; Eval Orig +} \GDGWords} \\
Cross-Attn + Obj-Centric & \bfseries 50.8 & \bfseries 49.3 & \bfseries 39.7 & \bfseries 30.6 \\
Cross-Attn + Patches & 46.2 & 45.5 & 30.5 & 14.8 \\
Concatenate + Obj-Centric & \uline{47.3} & \uline{47.3} & 32.0 & \uline{25.0} \\
Concatenate + Patches& 43.2 & 42.2 & \uline{32.5} & 19.6 \\
\bottomrule
\end{tabularx}
\caption{\textbf{Train Orig; Eval Orig. + GDG} Average success rates per level for each \GDG perturbation, demonstrating each model performing above random chance (0\%) despite lacking linguistic information. Per-task results are in \cref{app}.}
\label{tab:perf-gdg-on-orig}
\end{table}



==> tables/gdg.tex <==

\begin{table}[tb]
\centering
\footnotesize
\sisetup{table-format=2.1}
\renewcommand{\arraystretch}{1.25}
\begin{tabularx}{\linewidth}{X SSSS @{}}
\toprule
& {L1} & {L2} & {L3} & {L4} \\
\midrule
\multicolumn{5}{@{}l}{\textit{Trained on Original + }\GDGTokens} \\
Cross-Attn + Obj-Centric & \bfseries 57.9 & \uline{55.0} & \uline{39.1} & 16.9 \\
Cross-Attn + Patches & 44.3 & 40.9 & 29.6 & 11.4\\
Concatenate + Obj-Centric& \uline{55.9} & \bfseries 55.5 & \bfseries 42.0 & \bfseries 26.2 \\
Concatenate + Patches& 44.0 & 43.0 & 31.7 & \uline{21.6} \\

% \midrule[0.2pt] 
\multicolumn{5}{@{}l}{\textit{Trained on Original +} \GDGWords} \\
Cross-Attn + Obj-Centric & \bfseries 50.8 & \bfseries 49.3 & \bfseries 39.7 & \bfseries 30.6 \\
Cross-Attn + Patches & 46.2 & 45.5 & 30.5 & 14.8 \\
Concatenate + Obj-Centric & \uline{47.3} & \uline{47.3} & 32.0 & \uline{25.0} \\
Concatenate + Patches& 43.2 & 42.2 & \uline{32.5} & 19.6 \\
\midrule[0.2pt] 
\multicolumn{5}{@{}l}{\textit{Trained on Paraphrases + }\GDGTokens} \\
Cross-Attn + Obj-Centric & \bfseries 56.7 & \uline{54.5} & \uline{36.6} & \uline{22.9} \\
Cross-Attn + Patches & 45.2 & 45.9 & 34.0 & 15.1 \\
Concatenate + Obj-Centric  & \bfseries 56.7 & \bfseries 55.3 & \bfseries 45.8 & \bfseries 26.4 \\
Concatenate + Patches & 45.9 & 44.3 & 32.9 & 20.0 \\
% \midrule[0.2pt] 
\multicolumn{5}{@{}l}{\textit{Trained on Paraphrases +} \GDGWords} \\
Cross-Attn + Obj-Centric &  \bfseries 50.8 & \bfseries 51.8 & \bfseries 39.9 & \bfseries 33.8 \\
Cross-Attn + Patches &  \uline{46.7} & \uline{48.4} & 33.9 & 18.6 \\
Concatenate + Obj-Centric  &  44.8 & 44.5 & \uline{35.4} & \uline{23.9} \\
Concatenate + Patches & 44.3 & 42.7 & 31.0 & 19.0 \\
\bottomrule
\end{tabularx}
\caption{Average task success per level after applying each \GDG perturbation, showing all models outperforming random chance. Results are separated by training data: original instructions from \VIMABench (top) and paraphrases (bottom).}
\label{tab:perf-gdg}
\end{table}


==> tables/trained-without-instruct.tex <==
\begin{table}[tb]
\centering
\footnotesize
\sisetup{table-format=2.1}
\renewcommand{\arraystretch}{1.3}
\begin{tabularx}{\linewidth}{@{} X SSSS @{}}
\toprule
& {L1} & {L2} & {L3} & {L4} \\
\midrule
Cross-Attn + Obj-Centric & 0.3 & 0.2 & 0.3 & 0.2 \\
Cross-Attn + Patches & 51.5 & 51.0 & 37.7 & 15.9 \\
Concatenate + Obj-Centric  & 55.2 & 56.4 & 50.9 & 46.4 \\
Concatenate + Patches & 52.3 & 49.7 & 37.1 & 18.9 \\
\bottomrule
\end{tabularx}
\caption{Model Performance trained without instructions.}
\label{tab:perf-trained-without-instruct}
\end{table}


